Eclares: Energy-Aware Clarity-Driven Ergodic Search

Planning informative trajectories while considering the spatial distribution of the information over the environment, as well as constraints such as the robot's limited battery capacity, makes the long-time horizon persistent coverage problem complex. Ergodic search methods consider the spatial distribution of environmental information while optimizing robot trajectories; however, current methods lack the ability to construct the target information spatial distribution for environments that vary stochastically across space and time. Moreover, current coverage methods dealing with battery capacity constraints either assume simple robot and battery models, or are computationally expensive. To address these problems, we propose a framework called Eclares, in which our contribution is two-fold. 1) First, we propose a method to construct the target information spatial distribution for ergodic trajectory optimization using clarity, an information measure bounded between [0,1]. The clarity dynamics allows us to capture information decay due to lack of measurements and to quantify the maximum attainable information in stochastic spatiotemporal environments. 2) Second, instead of directly tracking the ergodic trajectory, we introduce the energy-aware (eware) filter, which iteratively validates the ergodic trajectory to ensure that the robot has enough energy to return to the charging station when needed. The proposed eware filter is applicable to nonlinear robot models and is computationally lightweight. We demonstrate the working of the framework through a simulation case study.

==> subsections/Definitions.tex <==
\newcommand{\norm}[1]{\left \| #1 \right \|}
\newcommand{\eqn}[1]{\begin{align}#1\end{align}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Pcal}{\mathcal{P}}

==> subsections/Extra.tex <==



% $\mathcal{S}^{n}_{+}$: symmetric positive-semidefinite matrices



















% Algorithm structure

\RestyleAlgo{ruled}
\LinesNumbered
\begin{algorithm}
\caption{Clarity-driven Ergodic Search}\label{alg:clarity}
\KwData{$n \geq 0$}
\KwResult{$y = x^n$}
$y \gets 1$\;
$X \gets x$\;
$N \gets n$\;
\While{$N \neq 0$}{
  \eIf{$N$ is even}{
    $X \gets X \times X$\;
    $N \gets \frac{N}{2}$ \Comment*[r]{This is a comment}
  }{\If{$N$ is odd}{
      $y \gets y \times X$\;
      $N \gets N - 1$\;
    }
  }
}
\end{algorithm}


% Figure with subfigures: (PROBLEM: Somehow when I use it, I end up having same figure number for two figures
% \begin{figure}[t]
%     \centering
%     \ContinuedFloat
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{media/Clarity_deficit_S.png}
%         \caption{Spatiostatic Environment}
%         \label{fig:S_ENV}
%     \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{media/Clarity_deficit_ST.png}
%         \caption{Stochastic Spatiotemporal Environment}
%         \label{fig:sto_ST_ENV}
%     \end{subfigure}
%     \caption{Caption for this figure with two images}
% \label{fig:image2}
% \end{figure}


% @ARTICLE{data_mpc,
%   author={Torrente, Guillem and Kaufmann, Elia and Föhn, Philipp and Scaramuzza, Davide},
%   journal={IEEE Robotics and Automation Letters}, 
%   title={Data-Driven MPC for Quadrotors}, 
%   year={2021},
%   volume={6},
%   number={2},
%   pages={3769-3776},
%   doi={10.1109/LRA.2021.3061307}}

% @ARTICLE{Panagou_sensing,
%   author={Panagou, Dimitra and Stipanović, Dušan M. and Voulgaris, Petros G.},
%   journal={IEEE Transactions on Control of Network Systems}, 
%   title={Distributed Dynamic Coverage and Avoidance Control Under Anisotropic Sensing}, 
%   year={2017},
%   volume={4},
%   number={4},
%   pages={850-862},
%   doi={10.1109/TCNS.2016.2576403}}

%   @article{hewing2019cautious,
%   title={Cautious model predictive control using gaussian process regression},
%   author={Hewing, Lukas and Kabzan, Juraj and Zeilinger, Melanie N},
%   journal={IEEE Transactions on Control Systems Technology},
%   volume={28},
%   number={6},
%   pages={2736--2743},
%   year={2019},
%   publisher={IEEE}
% }


% @inproceedings{sharma2020risk,
%   title={Risk-aware planning and assignment for ground vehicles using uncertain perception from aerial vehicles},
%   author={Sharma, Vishnu D and Toubeh, Maymoonah and Zhou, Lifeng and Tokekar, Pratap},
%   booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
%   pages={11763--11769},
%   year={2020},
%   organization={IEEE}
% }

% @article{hakobyan2019risk,
%   title={Risk-aware motion planning and control using CVaR-constrained optimization},
%   author={Hakobyan, Astghik and Kim, Gyeong Chan and Yang, Insoon},
%   journal={IEEE Robotics and Automation letters},
%   volume={4},
%   number={4},
%   pages={3924--3931},
%   year={2019},
%   publisher={IEEE}
% }

% @book{boyd1994linear,
%   title={Linear matrix inequalities in system and control theory},
%   author={Boyd, Stephen and El Ghaoui, Laurent and Feron, Eric and Balakrishnan, Venkataramanan},
%   year={1994},
%   publisher={SIAM}
% }

% @article{brady_cvar,
%   author       = {Arnav Choudhry and
%                   Brady G. Moon and
%                   Jay Patrikar and
%                   Constantine Samaras and
%                   Sebastian A. Scherer},
%   title        = {CVaR-based Flight Energy Risk Assessment for Multirotor UAVs using
%                   a Deep Energy Model},
%   journal      = {CoRR},
%   volume       = {abs/2105.15189},
%   year         = {2021},
%   url          = {https://arxiv.org/abs/2105.15189},
%   eprinttype    = {arXiv},
%   eprint       = {2105.15189},
%   timestamp    = {Wed, 02 Jun 2021 11:46:42 +0200},
%   biburl       = {https://dblp.org/rec/journals/corr/abs-2105-15189.bib},
%   bibsource    = {dblp computer science bibliography, https://dblp.org}
% }

% @inproceedings{richter2016polynomial,
%   title={Polynomial trajectory planning for aggressive quadrotor flight in dense indoor environments},
%   author={Richter, Charles and Bry, Adam and Roy, Nicholas},
%   booktitle={Robotics Research: The 16th International Symposium ISRR},
%   pages={649--666},
%   year={2016},
%   organization={Springer}
% }

@inproceedings{lee2010geometric,
  title={Geometric tracking control of a quadrotor UAV on SE (3)},
  author={Lee, Taeyoung and Leok, Melvin and McClamroch, N Harris},
  booktitle={49th IEEE conference on decision and control (CDC)},
  pages={5420--5425},
  year={2010},
  organization={IEEE}
}


% @inproceedings{mitchell2005toolbox,
%   title={A toolbox of Hamilton-Jacobi solvers for analysis of nondeterministic continuous and hybrid systems},
%   author={Mitchell, Ian M and Templeton, Jeremy A},
%   booktitle={International workshop on hybrid systems: computation and control},
%   pages={480--494},
%   year={2005},
%   organization={Springer}
% }


% @article{ocean1,
% title = "Multi-AUV control and adaptive sampling in Monterey Bay",
% author = "Edward Fiorelli and Leonard, {Naomi Ehrich} and Pradeep Bhatta and Paley, {Derek A.} and Ralf Bachmayer and Fratantoni, {David M.}",
% year = "2006",
% month = oct,
% doi = "10.1109/JOE.2006.880429",
% language = "English (US)",
% volume = "31",
% pages = "935--948",
% journal = "IEEE Journal of Oceanic Engineering",
% issn = "0364-9059",
% publisher = "Institute of Electrical and Electronics Engineers Inc.",
% number = "4",
% }

% @article{ocean2,
% author = {Curtin, Thomas and Bellingham, James},
% year = {2001},
% month = {11},
% pages = {421 - 423},
% title = {Guest editorial: Autonomous ocean-sampling networks},
% volume = {26},
% journal = {Oceanic Engineering, IEEE Journal of},
% doi = {10.1109/JOE.2001.972072}
% }

% @article{ocean3,
% author = {Leonard, Naomi and Paley, Derek and Lekien, Francois and Sepulchre, Rodolphe and Fratantoni, David and Davis, Russ},
% year = {2007},
% month = {01},
% pages = {48-74},
% title = {Collective Motion, Sensor Networks, and Ocean Sampling},
% volume = {95},
% journal = {Proceedings of the IEEE},
% doi = {10.1109/JPROC.2006.887295}
% }
% @inproceedings{xiao2019control,
%   title={Control barrier functions for systems with high relative degree},
%   author={Xiao, Wei and Belta, Calin},
%   booktitle={2019 IEEE 58th conference on decision and control (CDC)},
%   pages={474--479},
%   year={2019},
%   organization={IEEE}
% }

% @inproceedings{zhang2019beyond,
%   title={Beyond point clouds: Fisher information field for active visual localization},
%   author={Zhang, Zichao and Scaramuzza, Davide},
%   booktitle={2019 International Conference on Robotics and Automation (ICRA)},
%   pages={5986--5992},
%   year={2019},
%   organization={IEEE}
% }

% @inproceedings{jiang2015higher,
%   title={Higher order Voronoi based mobile coverage control},
%   author={Jiang, Bomin and Sun, Zhiyong and Anderson, Brian DO},
%   booktitle={2015 American Control Conference (ACC)},
%   pages={1457--1462},
%   year={2015},
%   organization={IEEE}
% }

% @inproceedings{hollinger2013sampling,
%   title={Sampling-based Motion Planning for Robotic Information Gathering.},
%   author={Hollinger, Geoffrey A and Sukhatme, Gaurav S},
%   booktitle={Robotics: Science and Systems},
%   volume={3},
%   number={5},
%   pages={1--8},
%   year={2013}
% }

% @INPROCEEDINGS{ener5,
%   author={Wei, Minghan and Isler, Volkan},
%   booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)}, 
%   title={Coverage Path Planning Under the Energy Constraint}, 
%   year={2018},
%   volume={},
%   number={},
%   pages={368-373},
%   doi={10.1109/ICRA.2018.8462867}}

%   @article{frontier_init,
%   title={A frontier-based approach for autonomous exploration},
%   author={Brian Yamauchi},
%   journal={Proceedings 1997 IEEE International Symposium on Computational Intelligence in Robotics and Automation CIRA'97. 'Towards New Computational Principles for Robotics and Automation'},
%   year={1997},
%   pages={146-151}
% }

% @INPROCEEDINGS{uzh_frontrier,
%   author={Cieslewski, Titus and Kaufmann, Elia and Scaramuzza, Davide},
%   booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, 
%   title={Rapid exploration with multi-rotors: A frontier selection method for high speed flight}, 
%   year={2017},
%   volume={},
%   number={},
%   pages={2135-2142},
%   doi={10.1109/IROS.2017.8206030}}

% @article{frontier_gradient,
%   author       = {Di Deng and
%                   Runlin Duan and
%                   Jiahong Liu and
%                   Kuangjie Sheng and
%                   Kenji Shimada},
%   title        = {Robotic Exploration of Unknown 2D Environment Using a Frontier-based
%                   Automatic-Differentiable Information Gain Measure},
%   journal      = {CoRR},
%   volume       = {abs/2011.05323},
%   year         = {2020},
%   url          = {https://arxiv.org/abs/2011.05323},
%   eprinttype    = {arXiv},
%   eprint       = {2011.05323},
%   timestamp    = {Thu, 12 Nov 2020 15:14:56 +0100},
%   biburl       = {https://dblp.org/rec/journals/corr/abs-2011-05323.bib},
%   bibsource    = {dblp computer science bibliography, https://dblp.org}
% }



% @article{persis_cbf2,
%   author       = {Gennaro Notomista and
%                   Magnus Egerstedt},
%   title        = {Persistification of Robotic Tasks},
%   journal      = {CoRR},
%   volume       = {abs/1903.05810},
%   year         = {2019},
%   url          = {http://arxiv.org/abs/1903.05810},
%   eprinttype    = {arXiv},
%   eprint       = {1903.05810},
%   timestamp    = {Sun, 31 Mar 2019 19:01:24 +0200},
%   biburl       = {https://dblp.org/rec/journals/corr/abs-1903-05810.bib},
%   bibsource    = {dblp computer science bibliography, https://dblp.org}
% }












% Consider continuous-time system dynamics comprising robot state dynamics and battery discharge dynamics:

% \begin{equation}
% \label{eqn:aug_ctrlaffine_sys}
%      \Dot{\chi} =
%     \begin{bmatrix}
%         \Dot{x} \\
%         \Dot{e} 
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%         f_r(x, u) \\
%         f_e(e, x, u) 
%     \end{bmatrix}
% \end{equation}
% % Throughout this paper, we use $x_r$ to refer to the robot state and $x$ to refer to the system state.
% where  $\chi = \begin{bmatrix}{x}^T, & e\end{bmatrix}^T \in  \mathbb{R}^{n+1}$ is the system state vector consisting of the robot's nominal state vector $x \in \mathcal{X} \subset \mathbb{R}^{n}$ and robot's state-of-charge (soc) $e \in \mathbb{R}_{\geq 0}$, $u \in \mathcal{U} \subset \mathbb{R}^{m}$ is the robot control input vector, $f_r: \mathbb{R}^n \times \mathbb{R}^m \rightarrow \mathbb{R}^n$ define continuous-time robot dynamics and $f_e: \mathbb{R}_{\geq 0} \rightarrow \mathbb{R}_{\geq 0}$ define continuous-time battery discharge dynamics. Given a control policy $\pi : [t_0, \infty) \times \mathcal{X} \rightarrow \mathcal{U}$ and an initial condition $x(t_0) = x_0$, the initial-value problem describing the closed-loop robot dynamics is:

% \begin{equation}
% \label{eqn:ctrlaffine_sys_control}
%  \Dot{x} = f_r(x, \pi(t,x)), \quad x(t_0)=x_0.
% \end{equation}

% Define a rectangular coverage space $\mathcal{P} \subset \mathbb{R}^{s}$ with dimension\footnote{If s=2, then coverage space is 2D and if s=3, then it is 3D.} $s$, such that $\mathcal{P} = [0,L_1] \times \cdots \times [0,L_s]$, where $L_i$ are the coverage space bounds and $s \leq n$. Let  $\Psi(x): \mathcal{X} \rightarrow \mathcal{P}$ be the mapping between state space $\mathcal{X}$ and coverage space $\mathcal{P}$. For example, if we have a 2D Euclidean coverage space i.e. $\mathcal{P} \subset \mathbb{R}^{2}$, then the mapping $\Psi(x)$ would convert robot state $x \in \mathbb{R}^{n}$ to a point $p \in \mathbb{R}^2$ in coverage space $\mathcal{P}$. Additionally, let's define $\phi: \mathcal{P} \rightarrow \mathbb{R}$ to be a target spatial distribution, where $\phi(p)$ is the density at a point $p \in \mathcal{P}$. The target spatial density $\phi(p)$ represents the target information density about a certain quantity of interest\footnote{For example, the salinity at the ocean surface.} at point $p$ in the coverage space $\mathcal{P}$.

% %\textbf{THIS DOES NOT MAKE SENSE. DO YOU CONSIDER THAT YOUR POLICY pi IN (2) IS AN ERGODIC CONTROLLER? AND READ WHAT YOU ARE WRITING: IN EFFECT YOU ARE SAYING "ERGODIC IS .... ERGODIC"} Ergodic search generates system trajectory $x(t; t_0, x_0), \forall t \in [t_0, T] $, as a solution to \eqref{eqn:ctrlaffine_sys_control}, that is \textit{ergodic} with respect to some target spatial distribution $\phi$. 
% Under a control policy $\pi:[t_0,\infty)\times \mathcal X\rightarrow \mathcal U$, the solution (trajectory) $x(t;t_0,x_0)$ of \eqref{eqn:ctrlaffine_sys_control} from initial state $x(t_0)=x_0$ is called ergodic with respect to a spatial distribution $\phi:\mathcal P\rightarrow \mathbb R$ if the time spent by the robot along the resulting trajectory at a point $p \in \mathcal{P}$ is proportional to the target spatial density $\phi(p)$ at point $p$ \cite{Dressel_Ergodic}. \textbf{UNCLEAR: AGAIN WHAT IS x(t)? WHAT IT MEANS TO SPEND TIME AT POINT? IS IT WITH ZERO SPEED? HOW CAN THIS BE DEFINED USING x(t)?}The proportion of the time spent by the robot at a particular point $p$ in $\mathcal{P}$ during the trajectory $x(t)$ is equal to the trajectory time-averaged statistics $c$ given as 

% \begin{equation}
%     c(p, x(t)) = \frac{1}{T} \int^{T}_{t_0} \delta(p - \Psi(x(t))))dt
% \end{equation}

% where $\delta$ is the Dirac delta function and $\Psi(\cdot)$ is the mapping between robot state at time $t$ during trajectory $x(t)$ and the point $p$ in coverage space $\mathcal{P}$. Ergodic search minimizes the difference between the Fourier coefficients of the spatial distribution $\phi$ and the trajectory time-averaged statistics $c$. For this purpose,~\cite{Mezic_Ergodic} proposed the ergodic metric 

% \begin{equation}
%     \label{eqn:ergodic_measure}
%     \Phi(x(t), \phi) = \sum_{k \in \mathcal{K}^s} \Lambda_k \|c_k - \phi_k\|^2
% \end{equation}
% where $k \in \mathcal{K}^s$ is the set of all fundamental frequencies, $c_k$, $\phi_k$ are the $k^{th}$ Fourier decomposition of $c$ and $\phi$ respectively, and $\Lambda_k = \frac{1}{(1 + ||k||^2)^{(s+1)/2}}$ is the scaling factor of the $k^{th}$ Fourier decomposition weighing low frequency features more heavily. An ergodic trajectory can be generated by formulating a trajectory optimization problem defined as 

% \begin{equation}
%     \label{eq:ergodic_optimzation_cont}
%     \begin{aligned}
%         \min_{x(t),u(t)} \quad & \{\Phi(x(t), \phi) + \int^{T}_{t_0} u(t)^T\mathbf{R}u(t)dt\}\\
%     \textrm{s.t.} \quad & \Dot{x} = f(x, u) \\
%     & x_{t_0} = x(t_0)   \\
%     \end{aligned}
% \end{equation}

% \textbf{CONFUSING NOTATION: WHY NOW f, x, u? IS THAT ROBOT u? SOMETHING ELSE? AND AS I READ I DON'T SEE THE POINT OF DEFINING (2). DO YOU REALLY NEED TO REFER TO A POLICY PI?}
% where $ \mathbf{R} \in S_{++}^{m}$ is a diagonal positive-definite matrix weighting control effort, and $x_{t_0}$ is the initial robot state at time $t_0$. There are a few methods \cite{Mezic_Ergodic, Dressel_Ergodic, dong2023time} to solve this problem. We use the method proposed by \cite{Dressel_Ergodic}. For brevity and details on implementation, see \cite{Dressel_Ergodic}. This work focuses on designing the target spatial distribution $\phi$ of a spatiotemporally varying environment for ergodic trajectory optimization. 






% In order to persistently monitor the environment, we iteratively solve the optimization problem \eqref{eq:ergodic_optimzation_cont} to generate $T_E$ horizon ergodic trajectories ($x_{t_1}^{T_E|1}, x_{t_2}^{T_E|2}, \cdots, x_{t_k}^{T_E|i}$) for the UAV, where $x_{t_k}^{T_E|i}$ is the solution to the $i^{th}$ optimization problem \eqref{eq:ergodic_optimzation_cont}, generated at time $t_k$ for horizon $T_E$. During this mission, the target spatial distribution $\phi$ of the environment must be updated before solving the $i^{th}$ optimization problem \eqref{eq:ergodic_optimzation_cont} to get the new trajectory $x_{t_k}^{T_E|i}$. Amidst this coverage mission, we face two main challenges:
% \begin{itemize}
%     \item[\RNum{1}.] How to effectively construct target spatial distribution $\phi$ before each iteration of the optimization problem \eqref{eq:ergodic_optimzation_cont} while considering the stochastic nature of the environment? 
%     % An effective construction would consider factors such as the possibility of information decay due to the lack of measurements of a stochastic quantity of interest $m$ and the maximum attainable information about the environment. 
%     \item[\RNum{2}.] How to ensure that the UAV has enough energy to follow nominal ergodic trajectories? UAVs have limited battery capacity and must be recalled back to the charging station when energy is about to deplete.
% \end{itemize}
% These are essentially two different challenges and therefore, we pose two different problem statements to solve them. However, it is evident how these two problems fall under the overall theme of energy-aware persistent coverage of a stochastic spatiotemporally varying environment. We now define two problem statements:


% \begin{prob}
% \label{prob:prob_ergodic}
% Design the target spatial distribution $\phi$ to represent a stochastic spatiotemporally varying environment given by~\eqref{eqn: quantity_of_interest} to be used when solving the ergodic trajectory optimization problem given by~\eqref{eq:ergodic_optimzation_cont}. The target spatial distribution $\phi$ should satisfy following properties:
% \begin{itemize}
%     \item[\RNum{1}.] It should incorporate information decay due to the stochastic evolution of the environment modelled using~\eqref{eqn: quantity_of_interest}.
%     \item[\RNum{2}.] It should quantify the maximum achievable information $\forall p_c \in \mathcal{P}_{cells}$.
% \end{itemize}
% \end{prob}

% \begin{prob} 
% \label{prob:prob_energy}
% Consider the system dynamics model~\eqref{eqn:aug_ctrlaffine_sys} and a nominal clarity-driven ergodic trajectory planner that generates the desired trajectory by solving \eqref{eq:ergodic_optimzation_cont}. Design an algorithm to track the desired ergodic trajectory $x_{t_k}^{T_E}$ while satisfying energy constraints. Mathematically, the problem can be posed as

% \begin{equation}
%     \label{eq:problem2_math}
%     \begin{aligned}
%         \max_{x(t),u(t)} \quad & \int_{t_k}^{t_k + T_E} \mathbb{I} \left( \| x(t) - x_{t_k}^{T_E}(t)\| \leq \delta \right)dt\\
%     \textrm{s.t.} \quad & x(t_k) = x_{t_k} \\
%     & \Dot{x} = f(x, u)   \\
%     & x_e(t) \geq x_{e_{min}}, \forall t \in [t_k, t_k + T_E]   \\
%     \end{aligned}
% \end{equation}
% \end{prob}

% where $\mathbb{I}$ is an indicator function and is defined as

% \begin{equation}
%     \mathbb{I}= 
%     \begin{cases} 
%         1 & \text{if} \hspace{0.1cm} \| x(t) - x_{t_k}^{T_E}(t)\| \leq \delta  \\
%         0 &  \text{otherwise}
%     \end{cases}  
% \end{equation}

% and $\delta$ is the maximum error allowed between the desired and final trajectory. Another approach to solve the energy-aware task persistence problem would be to directly incorporate energy constraints in \eqref{eq:ergodic_optimzation_cont}, but the non-convexity of the problem \eqref{eq:ergodic_optimzation_cont} implies that guaranteeing convergence and recursive feasibility is challenging. Therefore, we pose the energy-aware task persistence problem as a separate low-level problem. While solving \cref{prob:prob_energy}, we make following assumptions:

% \begin{assumption}
% The battery discharge dynamics given as part of system dynamics \eqref{eqn:aug_ctrlaffine_sys} are known or at least the worst-case scenario discharge dynamics are known.  
% \end{assumption}

% \begin{assumption}
% We don't consider environmental disturbances in this work; however, this can be easily incorporated into the trajectory generation process \cite{hewing2019cautious, data_mpc}.
% \end{assumption}

% \begin{assumption}
% Considering a static base station or charging station is a standard assumption in most of the robotic task persistence literature \cite{persis_cbf1, persis_cbf2, persis_cbf3, persis_cbf4, will2}. In this work, we also consider the case of the dynamic base station, which could be any moving mobile robot. However, we assume that the trajectory of the dynamic base station is known at all times.  
% \end{assumption}


% \begin{remark}
% \label{rem:stochasticity}
% It is important to note that the environment can be spatiotemporally varying but not stochastic. In that case, $m$ will evolve according to some known model and therefore, once the information about the quantity of interest $m(p)$ is gained at some $p \in \mathcal{P}$, its known dynamics can be used to get its value further in time resulting in no loss of information. However, in this work, we model $m$ as stochastic, and thus that results in information loss. 
% \end{remark}


% Consider the system dynamics~\eqref{eqn:aug_ctrlaffine_sys}. Given a control policy $\pi : [t_0, \infty) \times \mathcal{X} \rightarrow \mathcal{U}$ and an initial condition $x(t_0) = x_0$, the initial-value problem describing the closed-loop augmented system dynamics is:
% \begin{figure} [H]
%   \centering
%   \includegraphics[width=1.0\columnwidth]{media/Traj_Eware.png}
%   \caption{TBA}
%   \label{fig:traj_eware}
% \end{figure}
% \begin{equation}
% \label{eqn:ctrlaffine_sys_control}
%  \Dot{x} = f(x, \pi(t,x))
% \end{equation}

% We now state some useful definitions, the problem statement, and some assumptions we make while solving the problem. 

% \begin{defn}[\textbf{Forward Invariant}]A  set  $\mathcal{F} \subset \mathcal{X}$ is forward invariant  on $t_0$ for the closed-loop dynamics \eqref{eqn:ctrlaffine_sys_control} if $\forall$ $x(t_0) \in \mathcal{F}$, $x(t) \in \mathcal{F}$ $\forall t \geq t_0$. 

% \begin{remark}
% \label{rem:render_FI}
% A controller $\pi : [t_0, \infty) \times \mathcal{X} \rightarrow \mathcal{U}$ renders $\mathcal{F}$ forward invariant if $\mathcal{F}$ is forward invariant for closed-loop dynamics $\eqref{eqn:ctrlaffine_sys_control}$.
% \end{remark}
% \end{defn}

% \begin{defn} Let $\mathcal{E}$ be a time-invariant set, which contains all the states $x$ where the robot's soc is greater than the minimum SOC threshold $x_{e_{min}}$. The set $\mathcal{E}$ is given as follows:

% \begin{equation}
% \label{eqn:energy_set}
%     \mathcal{E} = \{x: x_e(t) \geq x_{e_{min}}\},\forall t \geq t_0
% \end{equation}
% \end{defn}

% \begin{defn} Let $\mathcal{C} \subset \mathcal{E}$ be a time-invariant set, which contains all the states $x$ from where the minimum soc, $\Gamma(x(t))$, required to come back to the base station is less than the current soc. The set $\mathcal{C}$ is given as follows:

% \begin{equation}
% \label{eqn:min_energy_set}
%     \mathcal{C} = \{x: \Gamma(x(t)) \leq x_e(t) \},\forall t \geq t_0
% \end{equation}
% \end{defn}


% \begin{prob} 
% \label{prob:prob_energy}
% Consider the system dynamical system~\eqref{eqn:aug_ctrlaffine_sys} and a nominal clarity-driven ergodic trajectory planner that generates the desired trajectory by solving \eqref{eq:ergodic_optimzation_cont}. Design an algorithm to track the desired trajectory while rendering $\mathcal{C}$ forward invariant. 
% \end{prob}

% While solving \cref{prob:prob_energy}, we make following assumptions:

% \begin{assumption}
% The battery discharge dynamics given as part of system dynamics \eqref{eqn:aug_ctrlaffine_sys} are known or at least the worst-case scenario discharge dynamics are known.  
% \end{assumption}

% \begin{assumption}
% We don't consider environmental disturbances in this work; however, this can be easily incorporated into the trajectory generation process \cite{hewing2019cautious, data_mpc}.
% \end{assumption}

% \begin{assumption}
% Considering a static base station or charging station is a standard assumption in most of the robotic task persistence literature \cite{persis_cbf1, persis_cbf2, persis_cbf3, persis_cbf4, will2}. In this work, we also consider the case of the dynamic base station, which could be any moving mobile robot. However, we assume that the trajectory of the dynamic base station is known at all times.  
% \end{assumption}

%%%%%% ------------------------------------- Forward Invariance and related definitions ------------------------------- %%%%%%%%%%%%%%%%
% Before stating the problem statements, we first provide some definitions:

% \begin{defn}[\textbf{Forward Invariant}]A  set  $\mathcal{F} \subset \mathcal{X}$ is forward invariant  on $t_0$ for the closed-loop dynamics \eqref{eqn:ctrlaffine_sys_control} if $\forall$ $x(t_0) \in \mathcal{F}$, $x(t) \in \mathcal{F}$ $\forall t \geq t_0$. 
% \end{defn}

% \begin{remark}
% \label{rem:render_FI}
% A controller $\pi : [t_0, \infty) \times \mathcal{X} \rightarrow \mathcal{U}$ renders $\mathcal{F}$ forward invariant if $\mathcal{F}$ is forward invariant for closed-loop dynamics $\eqref{eqn:ctrlaffine_sys_control}$.
% \end{remark}

% \begin{figure} [t]
%   \centering
%   \includegraphics[width=1.0\columnwidth]{media/Sets_Eware.png}
%   \caption{Visual representation of sets $\mathcal{E}$~\eqref{eqn:energy_set} and $\mathcal{C}$~\eqref{eqn:min_energy_set} is shown here. The line $\Gamma(x)$ represents the minimum energy required to go back to the base station from any system state $x \in \mathcal{X}$.}
%   \label{fig:set_eware}
% \end{figure}
% \begin{defn} Considering system \eqref{eqn:aug_ctrlaffine_sys}, let $\mathcal{E}$ be a time-invariant set, which contains all the states $x$ where the robot's state-of-charge (soc) is greater than the minimum soc threshold $x_{e_{min}}$. The set $\mathcal{E}$ is given as follows:

% \begin{equation}
% \label{eqn:energy_set}
%     \mathcal{E} = \{x | x_e(t) \geq x_{e_{min}}\},\forall t \geq t_0
% \end{equation}
% \end{defn}



% \begin{defn} Considering system \eqref{eqn:aug_ctrlaffine_sys}, let $\mathcal{C} \subset \mathcal{E}$ be a time-invariant minimum-energy set, which contains all the states $x$ from where the minimum soc, $\Gamma(x(t))$, required to come back to the base station is less than the current soc. The set $\mathcal{C}$ is given as follows:

% \begin{equation}
% \label{eqn:min_energy_set}
%     \mathcal{C} = \{x | \Gamma(x(t)) \leq x_e(t) \},\forall t \geq t_0
% \end{equation}
% \end{defn}

% \cref{fig:set_eware} shows the visual representation of the set $\mathcal{E}$ and set $\mathcal{C}$. We now state the problem statements. 
%%%%%% ------------------------------------- Forward Invariance and related definitions ------------------------------- %%%%%%%%%%%%%%%%






@INPROCEEDINGS{TIGRIS,
  author={Moon, Brady and Chatterjee, Satrajit and Scherer, Sebastian},
  booktitle={2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, 
  title={TIGRIS: An Informed Sampling-based Algorithm for Informative Path Planning}, 
  year={2022},
  volume={},
  number={},
  pages={5760-5766},
  doi={10.1109/IROS47612.2022.9981992}}



  @inproceedings{ayvali2017ergodic,
  title={Ergodic coverage in constrained environments using stochastic trajectory optimization},
  author={Ayvali, Elif and Salman, Hadi and Choset, Howie},
  booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={5204--5210},
  year={2017},
  organization={IEEE}
}


@INPROCEEDINGS{will1,
  author={Bentz, William and Panagou, Dimitra},
  booktitle={2017 International Conference on Unmanned Aircraft Systems (ICUAS)}, 
  title={3D dynamic coverage and avoidance control in power-constrained UAV surveillance networks}, 
  year={2017},
  volume={},
  number={},
  pages={1-10},
  doi={10.1109/ICUAS.2017.7991388}}


@article{cao2013multi,
  title={Multi-robot informative path planning for active sensing of environmental phenomena: A tale of two algorithms},
  author={Cao, Nannan and Low, Kian Hsiang and Dolan, John M},
  journal={arXiv preprint arXiv:1302.0723},
  year={2013}
}

@INPROCEEDINGS{Rus_Daniela_persist,
  author={Smith, Stephen L. and Schwager, Mac and Rus, Daniela},
  booktitle={2011 IEEE International Conference on Robotics and Automation}, 
  title={Persistent monitoring of changing environments using a robot with limited range sensing}, 
  year={2011},
  volume={},
  number={},
  pages={5448-5455},
  doi={10.1109/ICRA.2011.5980251}}

  @article{kalman,
    Author = {Kalman, Rudolph Emil},
    Title = {A New Approach to Linear Filtering and Prediction Problems},
    Journal = {Transactions of the ASME--Journal of Basic Engineering},
    Volume = {82},
    Number = {Series D},
    Pages = {35--45},
    Year = {1960}
}@article{will3,
title = {A hybrid approach to persistent coverage in stochastic environments},
journal = {Automatica},
volume = {109},
pages = {108554},
year = {2019},
issn = {0005-1098},
doi = {https://doi.org/10.1016/j.automatica.2019.108554},
url = {https://www.sciencedirect.com/science/article/pii/S0005109819304157},
author = {William Bentz and Dimitra Panagou},
keywords = {Coverage control, Collision avoidance, Autonomous mobile robots, Cooperative control, Multi-agent systems},
}



% @ARTICLE{Fuel,
%   author={Zhou, Boyu and Zhang, Yichen and Chen, Xinyi and Shen, Shaojie},
%   journal={IEEE Robotics and Automation Letters}, 
%   title={FUEL: Fast UAV Exploration Using Incremental Frontier Structure and Hierarchical Planning}, 
%   year={2021},
%   volume={6},
%   number={2},
%   pages={779-786},
%   doi={10.1109/LRA.2021.3051563}}




@inproceedings{NicRoyQP,
  title={Polynomial Trajectory Planning for Aggressive Quadrotor Flight in Dense Indoor Environments},
  author={Charles Richter and Adam Bry and Nicholas Roy},
  booktitle={International Symposium of Robotics Research},
  year={2016},
  url={https://api.semanticscholar.org/CorpusID:9070368}
}

% ---------------------------------------------- Reachability Gramian Based Approach  (For arxiv version) ---------------------------------------------------
% \subsection{Reachability Gramian-based method for Linear Systems}

% In this method, I am talking about how Reachability gramian based technique is one of the methods to quantify how much energy is required to travel back to the charging station\cite{boyd1994linear}

% Assume that the system given by (1) is reachable, 

% \begin{equation}
% \label{eqn:lin_sys}
%  \Dot{x} = Ax + Bu
% \end{equation}


% we seek to minimize u that steers $x(0) = 0$ to $x(t) = x_{des}$ as shown below.
% \begin{equation}
%     \mathcal{E}_{min} = \min_{u(\tau)} \int_{0}^{t_f} ||u(\tau)||^2 d\tau
% \end{equation}

% The analytic expression for least-norm or minimum-energy control input is given as follows:

% \begin{equation}
%     \mathcal{E}_{min} = \int_{0}^{t_f}||u_{ln}(\tau)||^2 d\tau = x_{des}^{T}W_r(t_f)^{-1}x_{des}
% \end{equation}

% where $W_r(t_f)$ is the controllability gramian for system shown in \eqref{eqn:lin_sys} and given as follows:

% \begin{equation}
%     \label{eqn:gramian}
%     W_r(t_f) = \int_{0}^{f} e^{A\tau}BB^{T}e^{A^{T}\tau}d\tau
% \end{equation}

% Similarly, the least-norm continuous time input at time step $\tau$ is given as follows:

% \begin{equation}
%     u_{ln}(\tau) = B^{T}e^{A^{T}(t_f - \tau)} \left( \int_{0}^{t_f} e^{A\Bar{t}}BB^{T}e^{A^{T}\Bar{t}}d\Bar{t}\right)^{-1} x_{des}
% \end{equation}

% \RestyleAlgo{ruled}
% % \vspace{-5em}

% \begin{algorithm}[tb]
% \caption{The Generate-TSD algorithm}\label{alg:eclares}
% \KwData{Target clarity $\overline{q}$, Environment model \eqref{eqn: quantity_of_interest}}
% \KwResult{Clarity-based target spatial distribution $\phi$}
% Get clarity $q(t_0)$ at initial time $t_0$ using \eqref{eqn:clarity_dynamics_closed_form}\\
% Get $\phi$ using \eqref{eq:proposed_heuristic} based on $\overline{q}$ and $q(t_0)$\\
% Solve problem \eqref{eq:ergodic_optimzation_cont} to determine $x^{ergo, T_E}_{0}$ using $\phi$\ over the time interval $[t_0, t_0 + T_E]$\\
% $t_k \gets t_0$\\
% \While{$t_k < (t_0 + T_E)$}{
%     Solve the initial value problem \eqref{eqn:candidate} to determine $x^{can, T_C}_{k} (t)$ over the interval $[t_k, t_k + T_C]$\\
%     {\eIf{$x^{can, T_C}_{k} (t)$ is valid by \cref{defn:valid_condition_def}}{
%       $x^{com, T_C}_{k} (t)$ = $x^{can, T_C}_{k} (t)$\\
%     }
%     {
%         $x^{com, T_C}_{k} (t)$ = $x^{com, T_C}_{k - 1} (t)$
%         \algorithmiccomment{Here robot returns to the charging station}\\
%         \textbf{break}\\
%     }
%     }
%     $t_k \gets t_k + dt$
% }
% \end{algorithm}


% \begin{itemize}
%     \item every $T_H$ seconds, 
%     \begin{itemize}
%         \item Recompute a target spatial distribution $\phi$ using $\genTSD$($q_{p_c}(t_k)$, $\overline{q}_{p_c}$, $\Dot{m}_{p_c}$), where $q_{p_c}(t_k)$ is the clarity at the current time $t_k$ and $\overline{q}_{p_c}$ is the target clarity $\forall p_c \in \mathcal{P}_{cells}$, and $\Dot{m}_{p_c}$ is the environment model \eqref{eqn: quantity_of_interest}. 
%         \item Recompute the ergodic trajectory $x^{ergo, T_H}_{k}$ at state $x_k$ for time horizon $T_H$ using \texttt{PTO}($\phi$). 
%     \end{itemize}
%     \item every $T_E$ seconds, 
%     \begin{itemize}
%         \item Generate $x^{nom, T_N}_{k}$ over the time interval $[t_k, t_k + T_N]$
%         \item Generate $x^{b2b, T_N}_{n}$ over time interval $[t_n, t_n + T_B]$, where $t_n = t_k + T_N$
%         \item Solve initial-value problem \eqref{eqn:candidate} to determine $x^{can, T_C}_{k}$ over time interval $[t_k, t_k + T_C]$
%         \item Recompute the committed trajectory $x^{ergo, T_C}_{k}$ at state $x_k$ for time horizon $T_C$ using \texttt{eware}(), where $T_C < T_H$
%     \end{itemize}
% \end{itemize}


% The eware algotithm (1)
% \begin{algorithm}
% \caption{The $\eware$ filtering algorithm}\label{alg:eware}
% \begin{algorithmic}[1]
% % \Require System candidate trajectory $\chi^{can, T_C}_{k}$ defined over $[t_k, t_k + T_C]$ and minimum energy allowed for the robot $e_{min}$
% % \Ensure Robot committed trajectory $x^{com, T_C}_{k}$ defined over $[t_k, t_k + T_C]$
% \Function{$\eware$}{$e^{can, T_C}_{k}$, $x^{can, T_C}_{k}$, $e_{min}$}
%     \If{$e^{can, T_C}_{k}  (t) \geq e_{min}, \hspace{0.1cm} \forall t \in [t_k, t_k + T_C]$}
%         \State $x^{com, T_C}_{k}$ = $x^{can, T_C}_{k}$
%     \Else
%         \State $x^{com, T_C}_{k}$ = $x^{com, T_C}_{k-1}$
%     \EndIf
%     \State \Return $x^{com, T_C}_{k}$
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% We now define how to construct a candidate trajectory. Suppose at the time $t = t_k$
% \begin{itemize}
%     \item the robot state is $x(t_k) = x_k$
%     \item the robot nominal trajectory $x^{nom, T_N}_{k}$ defined over time interval $[t_k, t_k + T_N]$ is the portion of the high-level ergodic trajectory $x^{ergo, T_H}_{k}$ where $T_N$ is the time horizon for nominal trajectory and $T_N \leq T_H$
%     \item the robot back-to-base (b2b) trajectory $x^{b2b, T_B}_{n}$ defined over time interval $[t_n, t_n + T_B]$, where $T_B$ is the time horizon for b2b trajectory and $t_n = t_k + T_N$
% \end{itemize}









@misc{Gulf_data,
    url = {https://ncss.hycom.org/thredds/ncss/grid/GOMl0.04/expt_32.5/2019/dataset.html},
    title={NCSS for Grids (Grid as Point Dataset)},
    note = {Accessed: 2023-07-13}
}

@inproceedings{lee2010geometric,
  title={Geometric tracking control of a quadrotor UAV on SE (3)},
  author={Lee, Taeyoung and Leok, Melvin and McClamroch, N Harris},
  booktitle={49th IEEE conference on decision and control (CDC)},
  pages={5420--5425},
  year={2010},
  organization={IEEE}
}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this section, we outline the notation used throughout the paper, provide an overview of the ergodic search methods, and introduce clarity as an information measure. 
\label{sec:prelim}
\subsubsection{\textbf{Notation}}Let $\naturals = \{ 0, 1, 2, ... \} $. Let $\mathbb{R}$, $\mathbb{R}_{\geq 0}$, $\mathbb{R}_{> 0}$ be the set of reals, non-negative reals, and positive reals respectively. Let $\mathcal{S}^{n}_{++}$ denote set of symmetric positive-definite in $\mathbb{R}^{n \times n}$. Let $\mathcal{N}(\mu, \Sigma)$ denote a normal distribution with mean $\mu$ and covariance $\Sigma \in \mathcal{S}^{n}_{++}$. The space of continuous functions $f: \Acal \to \Bcal$ is denoted $C(\Acal, \Bcal)$. The $Q \in \pd^{n}$ norm of a vector $x \in \R^n$ is denoted $\norm{x}_Q = \sqrt{x^T Q x}.$

\subsubsection{\textbf{Dynamics Model}}
Consider the continuous-time system dynamics comprising the robot and battery discharge dynamics:

\begin{equation}
\label{eqn:aug_ctrlaffine_sys}
     \Dot{\chi} =
    \begin{bmatrix}
        \Dot{x} \\
        \Dot{e} 
    \end{bmatrix}
    =
    f(\chi, u) \\
    =
    \begin{bmatrix}
        f_r(x, u) \\
        f_e(e, x, u) 
    \end{bmatrix}
\end{equation}
% Throughout this paper, we use $x_r$ to refer to the robot state and $x$ to refer to the system state.
where \textcolor{red}{ $\chi = \begin{bmatrix}{x}^T, & e\end{bmatrix}^T \in \Zcal \subset \R^{n+1}$} is the system state consisting of the robot's state $x \in \mathcal{X} \subset \mathbb{R}^{n}$ and robot's State-of-Charge (SoC) $e \in \mathbb{R}_{\geq 0}$. $u \in \mathcal{U} \subset \mathbb{R}^{m}$ is the control input, $f: \Zcal \times \Ucal \rightarrow \mathbb{R}^{n+1}$ defines the continuous-time system dynamics, $f_r: \Xcal \times \Ucal \rightarrow \mathbb{R}^n$ define robot dynamics and $f_e: \mathbb{R}_{\geq 0} \times \Xcal \times \Ucal \to  \mathbb{R}$ define battery discharge dynamics. 

% Given a control policy $\pi : [t_0, \infty) \times \mathcal{X} \rightarrow \mathcal{U}$ and an initial condition $x(t_0) = x_0$, the initial-value problem describing the closed-loop robot dynamics is:

% \begin{equation}
% \label{eqn:ctrlaffine_sys_control}
%  \Dot{x} = f_r(x, \pi(t,x)), \quad x(t_0)=x_0.
% \end{equation}

\subsubsection{\textbf{Ergodic Search}}

%\textcolor{blue}{1). Here, whenever I refer to the trajectory it is of the robot. 2) Secondly, the trajectory is a solution to the optimization problem posed in \eqref{eq:ergodic_optimzation_cont}, thus I have removed the PI policy. We have also changed the description of the ergodic search; Hopefully, this one makes more conceptual sense and also gives us a little bit more space :)}
\label{sec:prelim_ergodic}


Ergodic search~\cite{Mezic_Ergodic, Dressel_Ergodic} is a technique to generate trajectories $\xi: [t_0, T] \to \mathcal{X}$ that cover a rectangular domain  $\mathcal{P} = [0, L_1] \times \cdots [0, L_s] \subset \mathbb{R}^s$, matching a specified \emph{target spatial distribution} (TSD) $\phi : \Pcal \to \R$, where $\phi(p)$ is the density at $p \in \mathcal{P}$. 
More precisely, given a trajectory $\xi : [t_0, T] \to \Xcal$, the \emph{spatial distribution} of $\xi$ is defined as
\begin{equation}
    c(\xi, p) = \frac{1}{T-t_0}\int_{t_0}^{T} \delta(p - \Psi(\xi(t))) dt
\end{equation}
where $\delta: \Pcal \to \R$ is the Dirac delta function and $\Psi: \Xcal \to \Pcal$ is a mapping such that $\Psi(\xi(t))$ is the position of the robot at time $t$. In other words, given a trajectory $\xi(t)$, $c(\xi, p)$ represents the fraction of time the robot spends at a point $p \in \Pcal$ over the interval $[t_0, T]$. Then, the \emph{ergodicity} of $\xi$ wrt to a given \emph{target spatial distribution} $\phi : \Pcal \to \R$ is
\eqn{
\Phi(\xi, \phi) = \norm{ c(\xi, \cdot) - \phi(\cdot)}_{H^{-(s+1)/2}}
}
where $\norm{\cdot}_{H^{-(s+1)/2}}$ is the Sobolev space norm defined in~\cite{Mezic_Ergodic}, i.e., $\Phi$ is a function space norm measuring the difference between the target spatial distribution $\phi(\cdot)$ and the spatial distribution of the trajectory $c(\xi, \cdot)$. In~\cite{Dressel_Ergodic} a Projection-based Trajectory Optimization (PTO) method is proposed to generate ergodic trajectories. It optimizes (over the space of trajectories $\xi \in C([t_0, T], \Xcal), u \in C([t_0, T], \Ucal)$)
\begin{equation}
    \label{eq:ergodic_optimzation_cont}
    \begin{aligned}
    \min_{\xi, u} \quad & \Bigl[\Phi(\xi, \phi) + J_b(\xi) + \int^{T}_{t_0} \norm{u(t)}^2 dt \Bigr]\\
    \textrm{s.t.} \quad & \Dot{x} = f(x, u) \\
    & x_{0} = x(t_0) 
    \end{aligned}
\end{equation}
where $J_b$ penalizes trajectories that leave the domain, and $x_{0}$ is the robot's state at $t_0$. The algorithm uses Fourier decompositions of $c, \phi$ to numerically evaluate $\Phi$ and its gradients with respect to $\xi, u$. This enables an efficient gradient descent algorithm to optimize \eqref{eq:ergodic_optimzation_cont}. In this paper, we do not modify the algorithm in~\cite{Dressel_Ergodic}. Instead, we focus on developing a strategy to systematically construct the target spatial distribution $\phi$ given the environment model and the robot's sensing model, as discussed later. 


\subsubsection{\textbf{Clarity}}
\label{sec:prelim_clarity}


Consider a stochastic variable (quantity of interest) $h\in \R$ governed by the process and output (measurement) models:
\begin{subequations}
\eqn{
    \Dot{h} &= w(t),   &&w(t) \sim \mathcal{N} (0, Q) \label{eqn: quantity_of_interest_point}\\ 
    y &= C(x)h+ v(t),  &&v(t) \sim \mathcal{N} (0, R)   \label{eqn: quantity_of_interest_measurement_point}
}
\end{subequations}
where $Q \in \Rnonneg$ is the known variance associated with the process noise, $y \in \R$ is the measurement, $C: \Xcal \to \R$ is the mapping between robot state and sensor state, and $R \in \R$ is the known variance of the measurement noise. %\textbf{DOES NOT MAKE SENSE: REMOVE OR REPHRASE:} If $h$ is estimated using Kalman Filter\cite{kalman} then in order to measure the quality of information possessed about a variable $h$, \cite{clarity} proposed \textit{Clarity}. 

In \cite{clarity}, we introduced the notion of clarity $q$ of the random quantity $h$, which lies between $[0,1]$ and is defined such that $q = 0$ represents $h$ being unknown, and $q = 1$ corresponds to $h$ being completely known. The clarity dynamics for the subsystem \eqref{eqn: quantity_of_interest_point}, \eqref{eqn: quantity_of_interest_measurement_point} are given by \cite{clarity}
\begin{equation}
    \label{eqn:clarity_dynamics}
    \Dot{q} = \frac{C(x)^2}{R}(1 - q)^2 - Qq^2
\end{equation}
If $C(x) = C$ is constant, \eqref{eqn:clarity_dynamics} admits a closed-form solution for the initial condition $q(0) = q_0$:
\begin{equation}
    \label{eqn:clarity_dynamics_closed_form}
    q(t; q_0) = q_{\infty} \left(1 + \frac{2\gamma_1}{\gamma_2 + \gamma_3 e^{2kQt}} \right)
\end{equation}
where $q_{\infty} = k/(k+1)$,  $k = C/ \sqrt{QR}$, $\gamma_1 = q_{\infty} - q_0$, $\gamma_2 = \gamma_1(k-1)$, $\gamma_3 = (k-1)q_0 - k$.

Notice that as $t \to \infty$, $q(t; q_0) \to q_\infty \leq 1$ monotonically. Thus $q_\infty$ defines the maximum attainable clarity. Equation~\eqref{eqn:clarity_dynamics_closed_form} can be inverted to determine the time required to increase the clarity from $q_0$ to some $q_1$. This time is denoted $\Delta T: [0, 1]^2 \to \Rnonneg$:
\eqn{
\Delta T(q_0, q_1) = t \text{ s.t. } q(t, q_0) = q_1 \quad \text{for } q_1 \in [q_0, q_\infty) \label{eqn:clarity_dynamics_inverse}
}
% \eqn{
% \Delta T(q_0, q_1) = \begin{cases}
%     0 & \text{if } q_1 < q_0\\
%     t \text{ s.t. } q(t, q_0) = q_1 & \text{if } q_1 \in [q_0, q_{\infty})
%     \end{cases}
%     \label{eqn:clarity_dynamics_inverse}
% }
For $q_1 < q_0$, we set $\Delta T(q_0, q_1) = 0$. $\Delta T(q_0, q_1)$ is undefined for $q_1 \geq q_\infty$. 

% For $q_0 \leq \overline q < q_\infty$, ~\eqref{eqn:clarity_dynamics_closed_form} is invertible. Let $\Delta t = \Delta t(q_0, \overline q)$ be the time such that
% \eqn{
% q(0) = q_0, \ q(\Delta t) = \overline q, \  \eqref{eqn:clarity_dynamics}
% }

% Let $\overline{q}$ be the target clarity to be achieved and $\Delta t$ be the time taken to achieve target clarity $\overline{q}$ from the initial clarity $q_0$. $\Delta t$ can computed by solving \eqref{eqn:clarity_dynamics_closed_form}.
\vspace{-1mm}































% Discrete time version of the Ergodic Search
% Among a few methods to solve this problem \cite{Mezic_Ergodic}\cite{Dressel_Ergodic}, we use the Projection-based Trajectory Optimization (PTO) proposed by \cite{Dressel_Ergodic}. For implementation sake, discrete approximations of system dynamics~\eqref{eqn:nom_ctrlaffine_sys}, $\phi$, $c$, $\phi_k$, and $c_k$ are used.\footnote{Please check \cite{Dressel_Ergodic} for discrete approximations of $c$ and $c_k$} The coverage space $\mathcal{P}$ is discretized into a normalized uniform grid containing $\mathcal{P}_{cells}$ cells and satisfying $\sum_{p_c \in \mathcal{P}_{cells}} \phi(p_c)V_c = 1$, where $p_c$ is a discrete cell in coverage space $\mathcal{P}$ and $V_c$ is the size\footnote{The size of the cell is the width in 1D, an area in 2D, and volume in 3D.} of the cell. The optimization problem to optimize the $T$ horizon discrete trajectory $\tilde{\textbf{x}}^{t, T}_r$ is defined as

% \begin{equation}
%     \label{eq:ergodic_optimzation}
%     \begin{aligned}
%         \min_{\tilde{\textbf{x}}^{t, T}_r,\tilde{\textbf{u}}^{t, T}_r} \quad & J(\tilde{\textbf{x}}^{t, T}_r,\tilde{\textbf{u}}^{t, T}_r)\\
%     \textrm{s.t.} \quad & \tilde{x}_{r, n+1} = \tilde{x}_{r, n} + f(\tilde{x}_{r, n}, \tilde{u}_n)\Delta t, \\
%     & n = 0, \cdots , N-1\\
%     & \tilde{x}_{r,0} = \tilde{x}_r(0)   \\
%     \end{aligned}
% \end{equation}

% where $\tilde{x}_{r, n} \in \mathcal{X}$ is the discrete robot state vector at time step $n$ and $\tilde{u}_{n} \in \mathcal{X}$ is the discrete control input vector at time step $n$. The cost $J(\tilde{\zeta}, u)$ is given as follows:

% \begin{equation}
%     J(\tilde{\zeta}, u) = q\Phi(\tilde{\zeta}) + \frac{\Delta t}{2}\sum_{n = 0}^{N-1} \tilde{u}_n^TR\tilde{u}_n + J_b(\tilde{\zeta})
% \end{equation}
% where $q$ weighs the ergodic metric, $R$ weights the control input, and $J_b(\tilde{\zeta})$ is the boundary penalty to keep the robot within the boundary of the rectangular coverage space $\mathcal{P}$  given as 

% \begin{equation}
%     J_b(\tilde{\zeta}) = c_b \sum^N_{n = 1} \sum^s_{i = 2} (\max (\tilde{\zeta}_{n,i} - L_i, 0)^2 + \min (\tilde{\zeta}_{n,i}, 0)^2)
% \end{equation}































% Important extra don't remove 
% % and let $N$-step trajectory $\tilde{\textbf{x}}^{t, N}_r$ to be the discrete-time version of $\textbf{x}^{t, T}_r$, where $N = T/\Delta t$ and $\Delta t$ is 





% \Require Clarity $q_{p_c}$ $\forall p_c \in \mathcal{P}_{cells}$, Target clarity $\overline{q}_{p_c}$ $\forall p_c \in \mathcal{P}_{cells}$, and Environment model $\Dot{m}_{p_c}$ \eqref{eqn: quantity_of_interest}
% \Ensure Clarity-based target spatial distribution $\phi_{p_c}$ $\forall p_c \in \mathcal{P}_{cells}$ to be used in ergodic trajectory optimization

% \Require System candidate trajectory $\chi^{can, T_C}_{k}$ defined over $[t_k, t_k + T_C]$ and minimum energy allowed for the robot $e_{min}$
% \Ensure Robot committed trajectory $x^{com, T_C}_{k}$ defined over $[t_k, t_k + T_C]$

% is start constructing $\phi({p_c})$ by first finding the maximum attainable clarity $q_{\infty, p_c}$ at each cell $p_c \in \mathcal{P}_{cells}$ based on the environment model (Lines 3-4). Based on  $q_{\infty, p_c}$, target clarity values are adjusted to ensure that the target clarity $\overline{q}_{p_c}$ is not greater than equal to the maximum attainable clarity at each cell (Line 5). The small positive constant $\epsilon$ is subtracted to ensure that $q_{\infty, p_c} \geq \overline{q}_{p_c}$; otherwise, $\Delta t_{p_c}$ at cell $p_c \in \Pcal_{cells}$ tends to infinity. Then, we compute $\Delta t_{p_c}$, $\forall p_c \in \mathcal{P}_{cells}$, using \eqref{eqn:clarity_dynamics_closed_form}, which is the time taken for clarity $q_{p_c}(t_0)$ at initial time $t_0$ to acquire the target clarity $\overline{q}_{p_c}$ (Line 6). Then, we set the $\Delta t_{p_c}$ to the $\phi_{p_c}$ (Line 7). In order to ensure that $\sum_{p_c \in \mathcal{P}_{cells}} \phi_{p_c} = 1.0$, we normalize  $\phi_{p_c}$ as shown in Line 10. 

==> subsections/related_work.tex <==
\textcolor{red}{Section still under construction; Please SKIP to next section}

\subsection{Coverage Methods}

In this subsection, I will talk about the following methods
\begin{itemize}
    \item Frontier-based Methods \cite{frontier_init}\cite{uzh_frontrier}\cite{frontier_gradient}\cite{Fuel}
    \item Sampling-based method (TIGRIS) \cite{Fuel}\cite{TIGRIS}
    \item William's method \cite{will1}\cite{will2}\cite{will3}
    \item Ergodic Method \cite{Mezic_Ergodic}\cite{Dressel_Ergodic}\cite{dong2023time}
\end{itemize}

Then write a concluding paragraph on what our contribution is in this area and it improves upon previous methods
Most of the current ergodic search-based methods denote spatial information distribution as Gaussian distribution \cite{Dressel_Ergodic,dong2023time} or some of the recent work \cite{cmu_ergodic} uses Bayesian-update-based dynamic maps proposed by \cite{Candela_thesis} \textcolor{red}{check this ref again}. 

\subsection{Energy-aware robotic task persistence}

In this subsection, I will talk about the following methods
\begin{itemize}
    \item CBF-based methods \cite{ames2016control}\cite{persis_cbf1}\cite{persis_cbf2}\cite{persis_cbf3}\cite{persis_cbf4}
    \item William's work on energy aware and reachability \cite{will1}\cite{will2}\cite{will3}\cite{mitchell2005toolbox}\cite{bansal2017hamilton}
    \item Work on Joint optimization of energy-aware trajectories 
    \item Conditional Value-at-Risk (CVaR) based methods (mainly Brady's paper) \cite{sharma2020risk}\cite{hakobyan2019risk}\cite{brady_cvar}
\end{itemize}

Then write a concluding paragraph on what our contribution is in this area and it improves upon previous methods
